Is Parallel Programming Hard, And, If So, What Can You Do About It? (Release v2023.06.11a)

The purpose of this book is to help you program shared-memory parallel systems without risking your sanity. Nevertheless, you should think of the information in this book as a foundation on which to build, rather than as a completed cathedral. Your mission, if you choose to accept, is to help make further progress in the exciting field of parallel programming-progress that will in time render this book obsolete. Parallel programming in the 21st century is no longer focused solely on science, research, and grand-challenge projects. And this is all to the good, because it means that parallel programming is becoming an engineering discipline. Therefore, as befits an engineering discipline, this book examines specific parallel-programming tasks and describes how to approach them. In some surprisingly common cases, these tasks can be automated. This book is written in the hope that presenting the engineering discipline underlying successful parallel-programming projects will free a new generation of parallel hackers from the need to slowly and painstakingly reinvent old wheels, enabling them to instead focus their energy and creativity on new frontiers. However, what you get from this book will be determined by what you put into it. It is hoped that simply reading this book will be helpful, and that working the Quick Quizzes will be even more helpful. However, the best results come from applying the techniques taught in this book to real-life problems. As always, practice makes perfect. But no matter how you approach it, we sincerely hope that parallel programming brings you at least as much fun, excitement, and challenge that it has brought to us!

==> memalloc/memalloc.tex <==
% memalloc/memalloc.tex
% mainfile: ../perfbook.tex
% SPDX-License-Identifier: CC-BY-SA-3.0

\chapter{Memory Allocation}
\label{chp:Memory Allocation}

High speed memory allocation as a case study for SMP design.

NCM's and paulmck/jacks's stuff from 1993, and later paper.

Bonwick stuff from 1994, and his later paper.

Spraul stuff from Linux.

